Stable deep neural network architectures for mitochondria segmentation on electron microscopy volumes

Electron microscopy (EM) allows the identification of intracellular organelles such as mitochondria, providing insights for clinical and scientific studies. In recent years, a number of novel deep learning architectures have been published reporting superior performance, or even human-level accuracy, compared to previous approaches on public mitochondria segmentation datasets. Unfortunately, many of these publications do not make neither the code nor the full training details public to support the results obtained, leading to reproducibility issues and dubious model comparisons. For that reason, and following a recent code of best practices for reporting experimental results, we present an extensive study of the state-of-the-art deep learning architectures for the segmentation of mitochondria on EM volumes, and evaluate the impact in performance of different variations of 2D and 3D U-Net-like models for this task. To better understand the contribution of each component, a common set of pre- and post-processing operations has been implemented and tested with each approach. Moreover, an exhaustive sweep of hyperparameters values for all architectures have been performed and each configuration has been run multiple times to report the mean and standard deviation values of the evaluation metrics. Using this methodology, we found very stable architectures and hyperparameter configurations that consistently obtain state-of-the-art results in the well-known EPFL Hippocampus mitochondria segmentation dataset. Furthermore, we have benchmarked our proposed models on two other available datasets, Lucchi++ and Kasthuri++, where they outperform all previous works. The code derived from this research and its documentation are publicly available.

==> sections/tables/lucchi_final_table.tex <==
\begin{table}[]
\hspace{-1.6cm}
\begin{adjustbox}{max width=1.2\textwidth}
\begin{tabular}{rrrrrlrrrrlr}
\hline
\textbf{}                        & \phantom{abc} & \textbf{}                          & \phantom{abc} & \multicolumn{4}{c}{\textbf{Foreground IoU}}                                                                                                    & \phantom{abc} & \multicolumn{3}{c}{\textbf{Overall IoU}}                                                                                     \\ \cline{5-8} \cline{10-12} 
                                 &               &                                    &               &                   & \multicolumn{1}{r}{\phantom{abc}} & \multicolumn{2}{c}{\textbf{50\% overlap}}                                              &               &                   & \multicolumn{1}{r}{\phantom{abc}} & \multicolumn{1}{c}{\textbf{50\% overlap}}                            \\ \cline{7-8} \cline{12-12} 
\textbf{Description}             &               & \textbf{Author}                    &               & \textbf{Reported} &                                   &                 & \textbf{\begin{tabular}[c]{@{}r@{}}+Ensemble\\ +Z-Fil.\end{tabular}} &               & \textbf{Reported} &                                   & \textbf{\begin{tabular}[c]{@{}r@{}}+Ensemble\\ +Z-Fil.\end{tabular}} \\ \hline
MultiResUNet                     &               & \cite{ibtehaz2020multiresunet}     &               & 0.847             &                                   & 0.814$\pm$0.014 & ~0.824$\pm$0.010                                                     &               & 0.919             &                                   & 0.902$\pm$0.007                                                      \\
2D network                       &               & Cheng~\cite{cheng2017volume}       &               & 0.865             &                                   & -               & -                                                                    &               & -                 &                                   & -                                                                    \\
3D Vanilla U-Net                 &               & \cite{cciccek20163d}               &               & 0.866             &                                   & 0.851$\pm$0.004 & 0.857$\pm$0.006                                                      &               & 0.929             &                                   & 0.924$\pm$0.003                                                      \\
Tiramisu                         &               & \cite{jegou2017one}                &               & 0.872             &                                   & 0.833$\pm$0.027 & 0.857$\pm$0.017                                                      &               & 0.932             &                                   & 0.924$\pm$0.009                                                      \\
2D U-Net                         &               & Casser~\cite{casser2020fast}       &               & 0.878             &                                   & -               & -                                                                    &               & 0.935             &                                   & -                                                                    \\
MNet                             &               & \cite{fu2018joint}                 &               & 0.883             &                                   & 0.865$\pm$0.008 & 0.874$\pm$0.007                                                      &               & 0.938             &                                   & 0.929$\pm$0.004                                                      \\
3D network                       &               & Cheng~\cite{cheng2017volume}       &               & 0.889             &                                   & -               & -                                                                    &               & -                 &                                   & -                                                                    \\
2D U-Net+Z-filtering             &               & Casser~\cite{casser2020fast}       &               & 0.890             &                                   & -               & -                                                                    &               & 0.942             &                                   & -                                                                    \\
FCN 8                            &               & \cite{dai2016r}                    &               & 0.893             &                                   & 0.880$\pm$0.003 & 0.888$\pm$0.002                                                      &               & 0.943             &                                   & 0.941$\pm$0.001                                                      \\
Working set + inference autostep &               & Lucchi~\cite{lucchi2014learning}   &               & 0.895             &                                   & -               & -                                                                    &               & 0.948             &                                   & -                                                                    \\
3D U-Net                         &               & Xiao~\cite{xiao2018automatic}      &               & 0.900             &                                   & -               & -                                                                    &               & -                 &                                   & -                                                                    \\
CNN+3 Post-proc.                 &               & Oztel~\cite{oztel2017mitochondria} &               & 0.907             &                                   & -               & -                                                                    &               & -                 &                                   & -                                                                    \\ \hline
3D SE U-Net                      &               & Ours                               &               & 0.879             &                                   & 0.867$\pm$0.009 & 0.874$\pm$0.007                                                      &               & 0.936             &                                   & 0.933$\pm$0.004                                                      \\
3D Attention U-Net               &               & Ours                               &               & 0.880             &                                   & 0.870$\pm$0.003 & 0.876$\pm$0.003                                                      &               & 0.936             &                                   & 0.934$\pm$0.002                                                      \\
2D Residual U-Net                &               & Ours                               &               & 0.885             &                                   & 0.873$\pm$0.005 & 0.880$\pm$0.004                                                      &               & 0.939             &                                   & 0.937$\pm$0.002                                                      \\
3D U-Net                         &               & Ours                               &               & 0.885             &                                   & 0.871$\pm$0.006 & 0.878$\pm$0.004                                                      &               & 0.939             &                                   & 0.935$\pm$0.002                                                      \\
3D Residual U-Net                &               & Ours                               &               & 0.888             &                                   & 0.877$\pm$0.004 & 0.883$\pm$0.002                                                      &               & 0.941             &                                   & 0.938$\pm$0.001                                                      \\
2D SE U-Net                      &               & Ours                               &               & 0.888             &                                   & 0.873$\pm$0.003 & 0.882$\pm$0.003                                                      &               & 0.941             &                                   & 0.937$\pm$0.002                                                      \\
2D U-Net                         &               & Ours                               &               & 0.893             &                                   & 0.881$\pm$0.002 & 0.888$\pm$0.002                                                      &               & 0.942             &                                   & 0.941$\pm$0.001                                                      \\
2D Attention U-Net               &               & Ours                               &               & 0.893             &                                   & 0.882$\pm$0.003 & 0.890$\pm$0.002                                                      &               & 0.943             &                                   & 0.942$\pm$0.001                                                      \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{Final scores obtained in Lucchi dataset. \textit{Z-Fil.} refers to Z-filtering, \textit{Ens.} to \textit{Ensemble} and \textit{MAX} to the maximum value among different runs. \textit{Reported} column refers to the final score reported by authors of different works. Thus, to compare our work we report also our best IoU/VOC values obtained: for our 2D networks the higher values are with +\textit{Smooth}+\textit{Z-Filtering}, and for 3D, with \textit{50\% Overlap}+\textit{Ensemble}.}
\end{table}

==> sections/tables/lucchi_final_table2.tex <==
{\centering\begin{sideways}
    \begin{minipage}{1\textheight}
        \resizebox{1\textheight}{!}{%
            \setstretch{1.2}

\begin{tabular}{rrrrrlrrrrlr}
\hline
\textbf{}                        & \phantom{abc} & \textbf{}                                   & \phantom{abc} & \multicolumn{4}{c}{\textbf{Foreground IoU}}                                                                                                             & \phantom{abc} & \multicolumn{3}{c}{\textbf{Overall IoU}}                                                                                     \\ \cline{5-8} \cline{10-12} 
                                 &               &                                             &               &                   & \multicolumn{1}{r}{\phantom{abc}} & \multicolumn{2}{c}{\textbf{50\% overlap}}                                                       &               &                   & \multicolumn{1}{r}{\phantom{abc}} & \multicolumn{1}{c}{\textbf{50\% overlap}}                            \\ \cline{7-8} \cline{12-12} 
\textbf{Description}             &               & \textbf{Author}                             &               & \textbf{\begin{tabular}[c]{@{}r@{}}Reported\\ (Maximum)\end{tabular}} &                                   &                          & \textbf{\begin{tabular}[c]{@{}r@{}}+Ensemble\\ +Z-Fil.\end{tabular}} &               & \textbf{Reported} &                                   & \textbf{\begin{tabular}[c]{@{}r@{}}+Ensemble\\ +Z-Fil.\end{tabular}} \\ \hline
FCN 32                           &               & \cite{dai2016r}                             &               & 0.688             &                                   & 0.677$\pm$0.005          & 0.680$\pm$0.006                                                      &               & 0.835             &                                   & 0.831$\pm$0.003                                                      \\
MultiResUNet                     &               & \cite{ibtehaz2020multiresunet}              &               & 0.847             &                                   & 0.814$\pm$0.014          & ~0.824$\pm$0.010                                                     &               & 0.919             &                                   & 0.902$\pm$0.007                                                      \\
2D network                       &               & Cheng~\cite{cheng2017volume}                &               & 0.865             &                                   & -                        & -                                                                    &               & -                 &                                   & -                                                                    \\
3D Vanilla U-Net                 &               & \cite{cciccek20163d}                        &               & 0.866             &                                   & 0.851$\pm$0.004          & 0.857$\pm$0.006                                                      &               & 0.929             &                                   & 0.924$\pm$0.003                                                      \\
Tiramisu                         &               & \cite{jegou2017one}                         &               & 0.872             &                                   & 0.833$\pm$0.027          & 0.857$\pm$0.017                                                      &               & 0.932             &                                   & 0.924$\pm$0.009                                                      \\
2D U-Net                         &               & Casser~\cite{casser2020fast}                &               & 0.878             &                                   & -                        & -                                                                    &               & 0.935             &                                   & -                                                                    \\
MNet                             &               & \cite{fu2018joint}                          &               & 0.883             &                                   & 0.865$\pm$0.008          & 0.874$\pm$0.007                                                      &               & 0.938             &                                   & 0.929$\pm$0.004                                                      \\
3D network                       &               & Cheng~\cite{cheng2017volume}                &               & 0.889             &                                   & -                        & -                                                                    &               & -                 &                                   & -                                                                    \\
2D U-Net+Z-filtering             &               & Casser~\cite{casser2020fast}                &               & 0.890             &                                   & -                        & -                                                                    &               & 0.942             &                                   & -                                                                    \\
FCN 8                            &               & \cite{dai2016r}                             &               & 0.893             &                                   & 0.880$\pm$0.003          & 0.888$\pm$0.002                                                      &               & 0.943             &                                   & 0.941$\pm$0.001                                                      \\
Working set + inference autostep &               & Lucchi~\cite{lucchi2014learning}            &               & 0.895             &                                   & -                        & -                                                                    &               & 0.948             &                                   & -                                                                    \\
3D U-Net                         &               & Xiao~\cite{xiao2018automatic}               &               & 0.900             &                                   & -                        & -                                                                    &               & -                 &                                   & -                                                                    \\
\textbf{CNN+3 Post-proc.}        & \textbf{}     & \textbf{Oztel~\cite{oztel2017mitochondria}} & \textbf{}     & \textbf{0.907}    & \textbf{}                         & \textbf{-}               & \textbf{-}                                                           & \textbf{}     & \textbf{-}        & \textbf{}                         & \textbf{-}                                                           \\ \hline
3D SE U-Net                      &               & Ours                                        &               & 0.879             &                                   & 0.867$\pm$0.009          & 0.874$\pm$0.007                                                      &               & 0.936             &                                   & 0.933$\pm$0.004                                                      \\
3D Attention U-Net               &               & Ours                                        &               & 0.880             &                                   & 0.870$\pm$0.003          & 0.876$\pm$0.003                                                      &               & 0.936             &                                   & 0.934$\pm$0.002                                                      \\
2D Residual U-Net                &               & Ours                                        &               & 0.885             &                                   & 0.873$\pm$0.005          & 0.880$\pm$0.004                                                      &               & 0.939             &                                   & 0.937$\pm$0.002                                                      \\
3D U-Net                         &               & Ours                                        &               & 0.885             &                                   & 0.871$\pm$0.006          & 0.878$\pm$0.004                                                      &               & 0.939             &                                   & 0.935$\pm$0.002                                                      \\
3D Residual U-Net                &               & Ours                                        &               & 0.888             &                                   & 0.877$\pm$0.004          & 0.883$\pm$0.002                                                      &               & 0.941             &                                   & 0.938$\pm$0.001                                                      \\
2D SE U-Net                      &               & Ours                                        &               & 0.888             &                                   & 0.873$\pm$0.003          & 0.882$\pm$0.003                                                      &               & 0.941             &                                   & 0.937$\pm$0.002                                                      \\
2D U-Net                         &               & Ours                                        &               & 0.893             &                                   & 0.881$\pm$0.002          & 0.888$\pm$0.002                                                      &               & 0.942             &                                   & 0.941$\pm$0.001                                                      \\
\textbf{2D Attention U-Net}      & \textbf{}     & \textbf{Ours}                               & \textbf{}     & \textbf{0.893}    & \textbf{}                         & \textbf{0.882$\pm$0.003} & \textbf{0.890$\pm$0.002}                                             & \textbf{}     & \textbf{0.943}    & \textbf{}                         & \textbf{0.942$\pm$0.001}                                             \\ \hline
\end{tabular}

}
        
        \captionof{table}{Final scores (mean$\pm$standard deviation) obtained in the Lucchi dataset. \textit{Z-Fil.} refers to \textit{Z-Filtering} and \textit{MAX} to the maximum value among different runs. \textit{Reported} column refers to the final score reported by authors of different works. Thus, to compare our work we report also our best foreground/overall IoU values obtained: for our 2D networks the higher values are with +\textit{Blended Ensemble}+\textit{Z-Filtering}, and for 3D, with \textit{50\% Overlap}+\textit{Ensemble}.}
\label{table:lucchi_final_table}
    \end{minipage}
\end{sideways}\par}

==> sections/tables/other_sota_network_table.tex <==
\begin{table}[]
\ra{1.2}
\hspace{-2.3cm}
\begin{adjustbox}{max width=1.4\textwidth}
\begin{tabular}{rrlrrrrrrrrrrrrrr}
\hline
\multicolumn{1}{c}{\textbf{}}                                                               & \multicolumn{1}{c}{\textbf{}}                                                & \multicolumn{1}{c}{\phantom{abc}} & \multicolumn{1}{c}{\textbf{}}                                 & \multicolumn{1}{c}{\phantom{abc}} & \multicolumn{4}{c}{\textbf{Per image}}                                                                                                       & \multicolumn{1}{c}{\phantom{abc}} & \multicolumn{3}{c}{\textbf{50\% Overlap}}                                                           & \multicolumn{1}{c}{\phantom{abc}} & \multicolumn{3}{c}{\textbf{Full Image}}                                                            \\ \cline{6-9} \cline{11-13} \cline{15-17} 
\textbf{Network}                                                                            & \textbf{\begin{tabular}[c]{@{}r@{}}Param.\\ number\\ (Million)\end{tabular}} &                                   & \textbf{\begin{tabular}[c]{@{}r@{}}Per \\ Patch\end{tabular}} &                                   & \textbf{}      & \textbf{+Z-Fil.} & \textbf{+Smooth} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}+Smooth\\ + Z-Fil.\end{tabular}}} &                                   & \textbf{}      & \textbf{+Ens.} & \textbf{\begin{tabular}[c]{@{}r@{}}+Ens.\\ +Z-Fil.\end{tabular}} &                                   & \textbf{}      & \textbf{+Ens.} & \textbf{\begin{tabular}[c]{@{}r@{}}+Ens.\\ +Z-Fil.\end{tabular}} \\ \hline
FCN 32~\cite{dai2016r}                                                                      & 50.381                                                                       &                                   & 0.040                                                         &                                   & 0.637          & 0.640            & 0.659           & 0.661                                                                                  &                                   & 0.677          & 0.679          & 0.680                                                            &                                   & 0.657          & 0.659          & 0.660                                                            \\
std                                                                                         & -                                                                            &                                   & 0.000                                                         &                                   & 0.005          & 0.005            & 0.003           & 0.003                                                                                  &                                   & 0.006          & 0.006          & 0.006                                                            &                                   & 0.003          & 0.003          & 0.003                                                            \\
MultiResUNet~\cite{ibtehaz2020multiresunet}                                                 & 7.26                                                                         &                                   & 0.815                                                         &                                   & 0.812          & 0.821            & 0.834           & 0.840                                                                                  &                                   & 0.814          & 0.820          & 0.824                                                            &                                   & 0.828          & 0.833          & 0.836                                                            \\
std                                                                                         & -                                                                            &                                   & 0.015                                                         &                                   & 0.016          & 0.015            & 0.010           & 0.009                                                                                  &                                   & 0.014          & 0.010          & 0.010                                                            &                                   & 0.016          & 0.010          & 0.014                                                            \\
Tiramisu~\cite{jegou2017one}                                                                & 9.4                                                                          &                                   & 0.810                                                         &                                   & 0.809          & 0.821            & 0.850           & 0.855                                                                                  &                                   & 0.833          & 0.851          & 0.857                                                            &                                   & 0.830          & 0.846          & 0.837                                                            \\
std                                                                                         & -                                                                            &                                   & 0.028                                                         &                                   & 0.030          & 0.029            & 0.016           & 0.016                                                                                  &                                   & 0.027          & 0.018          & 0.017                                                            &                                   & 0.029          & 0.019          & 0.029                                                            \\
Vanilla U-Net 3D~\cite{cciccek20163d}                                                       & 19.07                                                                        &                                   & 0.402                                                         &                                   & 0.842$(\dag)$  & 0.844$(\dag)$    & -               & -                                                                                      &                                   & 0.851          & 0.857          & 0.857                                                            &                                   & -              & -              & -                                                                \\
std                                                                                         & -                                                                            &                                   & 0.005                                                         &                                   & 0.004          & 0.005            & -               & -                                                                                      &                                   & 0.004          & 0.006          & 0.006                                                            &                                   & -              & -              & -                                                                \\
MNet~\cite{fu2018joint}                                                                     & 8.54                                                                         &                                   & 0.851                                                         &                                   & 0.854          & 0.861            & 0.874           & 0.878                                                                                  &                                   & 0.865          & 0.870          & 0.874                                                            &                                   & 0.867          & 0.872          & 0.873                                                            \\
std                                                                                         & -                                                                            &                                   & 0.011                                                         &                                   & 0.009          & 0.009            & 0.006           & 0.006                                                                                  &                                   & 0.008          & 0.007          & 0.007                                                            &                                   & 0.008          & 0.006          & 0.008                                                            \\
*U-Net 3D + SE~\cite{hu2018squeeze}                                                         & 0.79                                                                         &                                   & 0.387$(\dag)$                                                 &                                   & 0.854$(\dag)$  & 0.855$(\dag)$    & -               & -                                                                                      &                                   & 0.867          & 0.873          & 0.874                                                            &                                   & -              & -              & -                                                                \\
std                                                                                         & -                                                                            &                                   & 0.007                                                         &                                   & 0.013          & 0.013            & -               & -                                                                                      &                                   & 0.009          & 0.007          & 0.007                                                            &                                   & -              & -              & -                                                                \\
\begin{tabular}[c]{@{}r@{}}* U-Net 3D \\ + Attention~\cite{oktay2018attention}\end{tabular} & 0.797                                                                        &                                   & 0.389$(\dag)$                                                 &                                   & 0.856$(\dag)$  & 0.857$(\dag)$    & -               & -                                                                                      &                                   & 0.870          & 0.876          & 0.876                                                            &                                   & -              & -              & -                                                                \\
std                                                                                         & -                                                                            &                                   & 0.005                                                         &                                   & 0.003          & 0.003            & -               & -                                                                                      &                                   & 0.003          & 0.003          & 0.003                                                            &                                   & -              & -              & -                                                                \\
*U-Net 3D                                                                                   & \textbf{0.79}                                                                &                                   & 0.394$(\dag)$                                                 &                                   & 0.858$(\dag)$  & 0.859$(\dag)$    & -               & -                                                                                      &                                   & 0.871          & 0.878          & 0.878                                                            &                                   & -              & -              & -                                                                \\
std                                                                                         & -                                                                            &                                   & 0.005                                                         &                                   & 0.007          & 0.007            & -               & -                                                                                      &                                   & 0.006          & 0.004          & 0.004                                                            &                                   & -              & -              & -                                                                \\
*U-Net 2D + SE~\cite{hu2018squeeze}                                                         & 1.95                                                                         &                                   & 0.863                                                         &                                   & 0.861          & 0.869            & 0.880           & 0.883                                                                                  &                                   & 0.873          & 0.878          & 0.882                                                            &                                   & 0.875          & 0.881          & 0.881                                                            \\
std                                                                                         & -                                                                            &                                   & 0.002                                                         &                                   & 0.003          & 0.003            & 0.003           & 0.003                                                                                  &                                   & 0.003          & 0.003          & 0.003                                                            &                                   & 0.002          & 0.002          & 0.002                                                            \\
*Residual U-Net 2D                                                                          & 2.03                                                                         &                                   & 0.867                                                         &                                   & 0.864          & 0.871            & 0.878           & 0.882                                                                                  &                                   & 0.873          & 0.877          & 0.880                                                            &                                   & 0.875          & 0.877          & 0.880                                                            \\
std                                                                                         & -                                                                            &                                   & 0.005                                                         &                                   & 0.005          & 0.006            & 0.003           & 0.003                                                                                  &                                   & 0.005          & 0.004          & 0.004                                                            &                                   & 0.004          & 0.003          & 0.004                                                            \\
*Residual U-Net 3D                                                                          & 1.50                                                                         &                                   & 0.394$(\dag)$                                                 &                                   & 0.857$(\dag)$  & 0.858$(\dag)$    & -               & -                                                                                      &                                   & 0.877          & 0.883          & 0.883                                                            &                                   & -              & -              & -                                                                \\
std                                                                                         & -                                                                            &                                   & 0.004                                                         &                                   & 0.004          & 0.004            & -               & -                                                                                      &                                   & 0.004          & 0.002          & 0.002                                                            &                                   & -              & -              & -                                                                \\
FCN 8~\cite{dai2016r}                                                                       & 50.384                                                                       &                                   & 0.860                                                         &                                   & 0.864          & 0.871            & \textbf{0.887}  & \textbf{0.891}                                                                         &                                   & 0.880          & 0.884          & 0.888                                                            &                                   & 0.881          & 0.886          & 0.886                                                            \\
std                                                                                         & -                                                                            &                                   & 0.005                                                         &                                   & 0.005          & 0.005            & 0.002           & 0.002                                                                                  &                                   & 0.003          & 0.002          & 0.002                                                            &                                   & 0.003          & 0.002          & 0.003                                                            \\
*U-Net 2D                                                                                   & 1.95                                                                         &                                   & 0.874                                                         &                                   & 0.872          & 0.880            & 0.884           & 0.889                                                                                  &                                   & 0.881          & 0.884          & 0.888                                                            &                                   & 0.882          & 0.884          & 0.887                                                            \\
std                                                                                         & -                                                                            &                                   & 0.003                                                         &                                   & 0.003          & 0.003            & 0.002           & 0.002                                                                                  &                                   & 0.002          & 0.002          & 0.002                                                            &                                   & 0.003          & 0.002          & 0.003                                                            \\
\begin{tabular}[c]{@{}r@{}}* U-Net 2D \\ + Attention~\cite{oktay2018attention}\end{tabular} & 1.99                                                                         &                                   & \textbf{0.875}                                                &                                   & \textbf{0.873} & \textbf{0.882}   & 0.886           & \textbf{0.892}                                                                         &                                   & \textbf{0.882} & \textbf{0.885} & \textbf{0.890}                                                   &                                   & \textbf{0.884} & \textbf{0.886} & \textbf{0.890}                                                   \\
std                                                                                         & -                                                                            &                                   & 0.004                                                         &                                   & 0.003          & 0.003            & 0.001           & 0.001                                                                                  &                                   & 0.003          & 0.001          & 0.002                                                            &                                   & 0.002          & 0.001          & 0.002                                                            \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{IoU of other state-of-the-art and classic networks for semantic segmentation performance in Lucchi dataset. Different scores discussed in previous sections are shown, together with the post-processing methods adopted (\textit{Z-Fil.} refers to \textit{Z-Filtering} and \textit{Ens.} to \textit{Ensemble}). Notice again how the results vary depending on the merging method used. In 2D, the patch size is $256\:\mbox{pixels}\times256\:\mbox{pixels}$ while in 3D, $80\:\mbox{pixels}\times80\:\mbox{pixels}\times80\:\mbox{pixels}$ was used. In 3D, a minimum overlap (marked with $\dag$) was made to satisfy the shape defined: $3\:\mbox{pixels}\times1\:\mbox{pixels}\times37\:\mbox{pixels}$ in $x \times y \times z$ axis.}
\label{table:other_sota_networks}
\end{table}


==> sections/tables/sota_reproduced_papers.tex <==
\begin{table}[]
\ra{1.2}
\hspace{-2.4cm}
\begin{adjustbox}{max width=1.4\textwidth}
\begin{tabular}{rrrcrcrrrrcrrrcrrr}
\hline
\textbf{}                          & \textbf{}                                                                    &                                       & \phantom{abc} & \textbf{}                                                     & \phantom{abc} & \multicolumn{4}{c}{\textbf{Per Image}}                                                                                   & \phantom{abc} & \multicolumn{3}{c}{\textbf{50\% Overlap}}                                                      & \phantom{abc} & \multicolumn{3}{c}{\textbf{Full Image}}                                                       \\ \cline{7-10} \cline{12-14} \cline{16-18} 
\textbf{Network}                   & \textbf{\begin{tabular}[c]{@{}r@{}}Param.\\ number\\ (Million)\end{tabular}} & \multicolumn{1}{c}{\textbf{~Reported}} &               & \textbf{\begin{tabular}[c]{@{}r@{}}Per \\ Patch\end{tabular}} &               & \textbf{}     & \textbf{+Z-Fil.} & \textbf{+Smooth} & \textbf{\begin{tabular}[c]{@{}r@{}}+Smooth\\ +Z-Fil.\end{tabular}} &               & \textbf{} & \textbf{+Ens.} & \textbf{\begin{tabular}[c]{@{}r@{}}+Ens.\\ +Z-Fil.\end{tabular}} &               & \textbf{} & \textbf{+Ens.} & \textbf{\begin{tabular}[c]{@{}r@{}}+Ens.\\ +Z-Fil.\end{tabular}} \\ \hline
Cheng 2D~\cite{cheng2017volume}    & 0.6                                                                          & 0.865                                 &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
V0                                 & 0.59                                                                         &                                       &               & 0.503                                                         &               & 0.503         & 0.511            & 0.541            & 0.548                                                              &               & 0.517     & 0.517          & 0.521                                                            &               & 0.526     & 0.537          & 0.535                                                            \\
std                                & -                                                                            &                                       &               & 0.233                                                         &               & 0.233         & 0.238            & 0.250            & 0.254                                                              &               & 0.240     & 0.239          & 0.243                                                            &               & 0.244     & 0.244          & 0.249                                                            \\
V1                                 & 0.59                                                                         &                                       &               & 0.848                                                         &               & 0.843         & 0.852            & 0.865            & 0.871                                                              &               & 0.851     & 0.863          & 0.868                                                            &               & 0.853     & 0.865          & 0.861                                                            \\
std                                & -                                                                            &                                       &               & 0.012                                                         &               & 0.012         & 0.011            & 0.008            & 0.008                                                              &               & 0.011     & 0.010          & 0.010                                                            &               & 0.011     & 0.009          & 0.010                                                            \\
MAX                                & -                                                                            &                                       &               & 0.864                                                         &               & 0.858         & 0.865            & 0.878            & 0.883                                                              &               & 0.865     & 0.877          & 0.881                                                            &               & 0.865     & 0.878          & 0.870                                                            \\
                                   &                                                                              &                                       &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
Cheng 3D~\cite{cheng2017volume}    & 0.63                                                                         & 0.889                                 &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
V0                                 & 0.79                                                                         &                                       &               & 0.053$(\dag)$                                                 &               & 0.053$(\dag)$ & 0.053$(\dag)$    & -                & -                                                                  &               & 0.053     & 0.053          & 0.053                                                            &               & -         & -              & -                                                                \\
std                                & -                                                                            &                                       &               & 0.053                                                         &               & 0.053         & 0.053            & -                & -                                                                  &               & 0.053     & 0.053          & 0.053                                                            &               & -         & -              & -                                                                \\
V1                                 & 0.79                                                                         &                                       &               & 0.201                                                         &               & 0.208         & 0.210            & -                & -                                                                  &               & 0.215     & 0.247          & 0.247                                                            &               & -         & -              & -                                                                \\
std                                & -                                                                            &                                       &               & 0.201                                                         &               & 0.208         & 0.210            & -                & -                                                                  &               & 0.215     & 0.247          & 0.247                                                            &               & -         & -              & -                                                                \\
MAX                                & -                                                                            &                                       &               & 0.403                                                         &               & 0.417         & 0.420            & -                & -                                                                  &               & 0.429     & 0.493          & 0.494                                                            &               & -         & -              & -                                                                \\
                                   &                                                                              &                                       &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
Casser~\cite{casser2020fast}       & 1.96                                                                         & 0.890                                 &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
V0                                 & 1.94                                                                         &                                       &               & 0.566$(\dag)$                                                 &               & 0.560$(\dag)$ & 0.575$(\dag)$    & 0.597            & 0.606                                                              &               & 0.562     & 0.593          & 0.602                                                            &               & 0.562     & 0.596          & 0.576                                                            \\
std                                & -                                                                            &                                       &               & 0.296                                                         &               & 0.296         & 0.304            & 0.311            & 0.315                                                              &               & 0.297     & 0.308          & 0.312                                                            &               & 0.298     & 0.310          & 0.305                                                            \\
V1                                 & 1.94                                                                         &                                       &               & 0.814$(\dag)$                                                 &               & 0.812$(\dag)$ & 0.828$(\dag)$    & 0.843            & 0.852                                                              &               & 0.815     & 0.842          & 0.851                                                            &               & 0.817     & 0.845          & 0.832                                                            \\
std                                & -                                                                            &                                       &               & 0.047                                                         &               & 0.047         & 0.042            & 0.028            & 0.025                                                              &               & 0.044     & 0.029          & 0.025                                                            &               & 0.044     & 0.028          & 0.039                                                            \\
MAX                                & -                                                                            &                                       &               & 0.865                                                         &               & 0.864         & 0.876            & 0.870            & 0.877                                                              &               & 0.865     & 0.869          & 0.876                                                            &               & 0.867     & 0.867          & 0.878                                                            \\
                                   &                                                                              &                                       &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
Xiao~\cite{xiao2018automatic}      & 1.1                                                                          & 0.900                                 &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
V0                                 & 1.08                                                                         &                                       &               & 0.874$(\dag)$                                                 &               & 0.863$(\dag)$ & 0.864$(\dag)$    & -                & -                                                                  &               & 0.863     & 0.866          & 0.867                                                            &               & -         & -              & -                                                                \\
std                                & -                                                                            &                                       &               & 0.003                                                         &               & 0.004         & 0.004            & -                & -                                                                  &               & 0.004     & 0.004          & 0.004                                                            &               & -         & -              & -                                                                \\
V1                                 & 1.08                                                                         &                                       &               & 0.882$(\dag)$                                                 &               & 0.873$(\dag)$ & 0.874$(\dag)$    & -                & -                                                                  &               & 0.872     & 0.874          & 0.874                                                            &               & -         & -              & -                                                                \\
std                                & -                                                                            &                                       &               & 0.002                                                         &               & 0.003         & 0.003            & -                & -                                                                  &               & 0.003     & 0.003          & 0.003                                                            &               & -         & -              & -                                                                \\
MAX                                & -                                                                            &                                       &               & 0.885                                                         &               & 0.879         & 0.880            & -                & -                                                                  &               & 0.880     & 0.880          & 0.880                                                            &               & -         & -              & -                                                                \\
                                   &                                                                              &                                       &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
Oztel~\cite{oztel2017mitochondria} & -                                                                            & 0.907                                 &               &                                                               &               &               &                  &                  &                                                                    &               &           &                &                                                                  &               &           &                &                                                                  \\
V0                                 & 0.14                                                                         &                                       &               & 0.296                                                         &               & 0.411         & 0.424            & 0.424            & 0.427                                                              &               & 0.383     & 0.373          & 0.370                                                            &               & 0.114     & 0.051          & 0.098                                                            \\
std                                & -                                                                            &                                       &               & 0.003                                                         &               & 0.003         & 0.003            & 0.009            & 0.009                                                              &               & 0.005     & 0.011          & 0.012                                                            &               & 0.044     & 0.021          & 0.041                                                            \\
MAX                                & -                                                                            &                                       &               & 0.298                                                         &               & 0.413         & 0.426            & 0.438            & 0.442                                                              &               & 0.389     & 0.389          & 0.387                                                            &               & 0.055     & 0.019          & 0.040                                                            \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{IoU scores of reproduced state-of-the-art works in Lucchi dataset. Different scores discussed in previous sections are shown, together with the post-processing methods adopted (\textit{Z-Fil.} refers to \textit{Z-Filtering} and \textit{Ens.} to \textit{Ensemble}). Notice again how the results vary depending on the merging method used. \textit{V0} versions refer to exact configurations as reported by the authors. \textit{V1} corresponds to our best approach modifying \textit{V0} in some way to improve method's performance and results stability. The patch size and overlap (marked with $\dag$) in each work is as follows: 1) Cheng 2D patch $256\times256$, Cheng 3D subvolumes $128\times128\times96$ ($0\times0\times27$ overlap in $x\times y\times z$) ; 2) Casser patch $512\times512$ ($256\times0$ overlap in $x\times y$) ; 3) Xiao $448\times576\times20$ ($128\:\mbox{pixels}\times128\:\mbox{pixels}\times10\:\mbox{pixels}$ overlap in $x\times y\times z$) ; 4) Oztel, entire image used, $768\times1024$.}
\label{table:sota_reproduction}
\end{table}
